JWST COMPASS: NIRSpec/G395H Transmission Observations of the Super-Earth TOI-776b

We present two transit observations of the $\sim$520K, 1.85R$_\oplus$, 4.0M$_\oplus$ super-Earth TOI-776b with JWST NIRSpec/G395H, resulting in a 2.8-5.2$\mu$m transmission spectrum. Producing reductions using the ExoTiC-JEDI and Eureka! pipelines, we obtain a median transit depth precision of 34ppm for both visits and both reductions in spectroscopic channels 30 pixels wide ($\sim$0.02$\mu$m). We find that our independent reductions produce consistent transmission spectra, however, each visit shows differing overall structure. For both reductions, a flat line is preferred for Visit 1 while a flat line with an offset between the NRS1 and NRS2 detectors is preferred for Visit 2; however, we are able to correct for this offset during our modeling analysis following methods outlined in previous literature. Using picaso forward models, we can rule out metallicities up to at least 100$\times$ solar with an opaque pressure of 10$^{-3}$ bar to $\geq$3$\sigma$ in all cases, however, the exact lower limit varies between the visits, with Visit 1 ruling out $\lesssim$100$\times$ solar while the lower limits for Visit 2 extend beyond $\sim$350$\times$ solar. Our results add to the growing list of super-Earth atmospheric constraints by JWST, which provide critical insight into the diversity and challenges of characterizing terrestrial planets.

==> drafts.tex <==
%this paragraph here is now a whole new idea so we need to introduce it as such - either with a subsection header? or just a better easing in (probably the latter)
% I think by culling the opening sentence
% so I think this paragraph starts something like "though we obtain a variety of metallicity constraints between visits as previously seen in the literature (surely as previously seen SURELY), we find that one of the preferred scenarios is able to rule out metallicities to higher values than previously seen (cite papers)" basically a way to introduce that the 350-450x is kinda weird so like why is this thing so special and then it leads into the sentence "Despite the spread..." but without the despite the spread clause and say in particular it is different from compass analyses blah blah.
%The absolute spectra across visits and reductions differ by a median value of $\sim$13\,ppm, yet we find a difference of 100$\times$ solar between our \jedi and \eureka lower limit metallicities in Visit 1. %Despite the differences between reductions being on par with previous COMPASS targets, this spread in interpretation is also larger.


% we double checked to see if this is the case, see table 5?6?. we see that cantera and photochem obtain slightly different values for our 3sig lower limits at 1mbar. 
% a note in here about how this does not only apply to comparing values within this program as modelling set ups will not be completely identical between every study (see eg the no air papers which xy and bjorn who does ABC).
%%"when comparing analyses be careful that underlying chem network could be different even if radiative transfer is the same. see eg that other papers may have used eg cantera (cite)" blah
% so either that leads into the next sentence or the next paragraph? I think possible the next sentence becomes part of the next paragraph
%This again highlights that the interpretation of super-Earth atmospheres is highly model-dependent. 
%Teske \& Batalha et al., submitted, analyzing COMPASS target TOI-776c, also found significant differences in metallicity and compositional limits when comparing pure forward model interpolation against a nested sampling approach. 
%\citet{Asplund2009} for elemental (and thus solar) abundances.% (M/H=0.0191). %We note that our analysis therefore differs from previous COMPASS program works, which instead have used a \texttt{Cantera} chemical equilibrium solver \citep{Goodwin2022}, which in turn uses \citet{Lodders2009} abundances for metallicity and C/O ratio calculations  



% alright so we've dealt with "all models are a mess" but back to our rock, what the hell is going on
% though the cantera vs photochem difference can account for some of the elevation in constraint we obtain, even the cantera ones are still quite super solar, so do we find that in some cases the rock is so flat? maybe we don't have an answer but that can lead into this ending paragraph
